Convergence of the non-staggered Nessyahu-Tadmor scheme for coupled systems of one-dimensional nonlocal balance laws

We derive a second-order accurate, non-staggered central scheme based on the well-known Nessyahu-Tadmor scheme to approximate solutions of coupled systems of nonlocal balance laws. We show that the approximate solutions stay bounded by an exponential $L^\infty$ bound in time. Under linearity assumptions on the flux and source terms the approximate solutions converge weakly-$*$ to weak solutions of the nonlocal balance laws. Assuming stronger regularity, in particular on the convolution kernel, we show strong convergence towards entropy weak solutions in the nonlinear case. Numerical examples validate our results and demonstrate its applicability to various systems of nonlocal problems.

==> macros_arxiv.tex <==
\usepackage[english]{babel}  
% \usepackage[top=1.6in, bottom=1.6in, left=0.7in, right=0.7in]{geometry}
 \usepackage[left=20mm,right=20mm, top=23mm, bottom=23mm]{geometry}
% \setlength{\textwidth}{6in}
% \setlength{\textheight}{8.5in}
% \setlength{\oddsidemargin}{0in}
% \setlength{\evensidemargin}{0in}
% \setlength{\topmargin}{-0.5in}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathtools} % must be loaded
\usepackage{graphicx}
%\usepackage{a4wide}
\usepackage{verbatim}
\RequirePackage{ifthen}
\RequirePackage[T1]{fontenc}
\RequirePackage{amsthm}
\RequirePackage{color}
\RequirePackage{listings} 
\RequirePackage{epstopdf}
\RequirePackage{emptypage}
\RequirePackage[nolist]{acronym}
\RequirePackage{multirow}
\RequirePackage{enumerate,enumitem}
\RequirePackage{caption}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta}
\RequirePackage{latexsym,amscd,makeidx}
\RequirePackage{exscale}
\RequirePackage{mathrsfs}
\RequirePackage{hyperref}
\RequirePackage{url}
\RequirePackage{booktabs}
\RequirePackage{esdiff}
\RequirePackage{listings}
\RequirePackage{tabularx}
\RequirePackage[sort,numbers]{natbib}
\RequirePackage{verbatim}
\RequirePackage{comment}
%\RequirePackage{cite}
\RequirePackage{cleveref}
\crefname{equation}{}{}
\Crefname{Equation}{}{}
\usepackage{pgfplots} 
\usepackage{pgfgantt}
\usepackage{pdflscape}
\usepackage{bm}
%\usepackage[notref,notcite]{showkeys}
\pgfplotsset{compat=newest} 
\pgfplotsset{plot coordinates/math parser=false}
\numberwithin{equation}{section}
% Switch: Hide or show comments
	\newif\ifshowcomments								
%	\showcommentstrue				% show comments
	\showcommentsfalse				% hide comments


% Definition of environments
	\definecolor{mygrey}{gray}{0.65}
	
	% Detailed comments
	\ifshowcomments
		% Display comments in a specified environment
		\newenvironment{bcomment}[1][]
	 	{~\\~\\ \begin{color}{mygrey}\begin{small}\noindent\textbf{COMMENT: #1}~\\}
	 	{\end{small}\end{color}~\\~\\}
	\else
		% Hide comments
	 	\excludecomment{bcomment}
	\fi
	% Inline-Comments
	
	\ifshowcomments
		\newcommand{\scomment}[1]{{\color{mygrey} [#1]}}  % small comments within lines
	\else
		\newcommand{\scomment}[1]{\iffalse #1 \fi}
	\fi

% Adjust sign of a number for the tikz picture of the grid 
	\newcommand\checkindex[1]{
		\pgfmathsetmacro{\var}{#1}
		\pgfmathparse{ifthenelse(\var==0, "",ifthenelse(\var>0, "+#1","#1"))} \pgfmathresult}%

%For tikz plots
\newlength\fwidth

% Create 'todo' marker (called by \todo{TEXT})
\newcommand{\margtodo}
{\marginpar{\textbf{\textcolor{red}{ToDo}}}{}}
\newcommand{\todo}[1]
{{\textbf{\textcolor{red}{-- \margtodo{}#1 --}}}{}}

\newcommand{\margidea}
{\marginpar{\textbf{\textcolor{orange}{Idea}}}{}}
\newcommand{\idea}[1]
{{\textbf{\textcolor{orange}{-- \margidea{}#1 --}}}{}}

\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\BV}{BV}

\theoremstyle{plain}						% Default
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

%%%Notation:
%Define some shortcuts
%% math calligraphy
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%% math blackboard bold
%\newcommand{\A}{\mathbb{A}}
%\newcommand{\B}{\mathbb{B}}
%\newcommand{\C}{\mathbb{C}}
%\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
%\newcommand{\I}{\mathbb{I}}
%\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
%\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\T}{\mathbb{T}}
%\newcommand{\U}{\mathbb{U}}
%\newcommand{\V}{\mathbb{V}}
%\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}

%% New commands
\newcommand{\OAP}{$(\Omega,\mathcal{A},P)$}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
\newcommand{\sign}{\operatorname{sgn}}
\newcommand{\Div}{\operatorname{div}}
\newcommand{\lano}{\mathrm{o}}
\newcommand{\lanO}{\mathrm{O}}
\newcommand{\dint}{\displaystyle\int}
\newcommand{\dsup}{\displaystyle\sup}
\newcommand{\dsum}{\displaystyle\sum}
%\newcommand{\BV}{\operatorname{BV}}
\newcommand{\TV}{\operatorname{TV}}
\newcommand{\mm}{\operatorname{minmod}}
%System
\newcommand{\consys}{\cQ}

%Indicies
\newcommand\half{{\frac12}}
\newcommand\jmo{{j-1}}
\newcommand\jmh{{j-\half}}
\newcommand\jpmh{{j\pm\half}}
\newcommand\jph{{j+\half}}
\newcommand\jpo{{j+1}}
\newcommand{\jpk}{{j+k}}
\newcommand{\jpko}{{j+k+1}}
\newcommand{\kmo}{{k-1}}
\newcommand\npo{{n+1}}

%Step sizes
\newcommand{\Dx}{\Delta x}
\newcommand{\Dt}{\Delta t}

%Computations
\newcommand\dx{\mathit{dx}}
\newcommand\dy{\mathit{dy}}
\newcommand\dt{\mathit{dt}}
\newcommand\ds{\mathit{ds}}
\newcommand{\norm}[1]{{\left\|#1\right\|}}
\newcommand{\abs}[1]{{\left|#1\right|}}

%Spaces:
\newcommand{\LinfR}{{L^\infty(\R)}}
\newcommand{\LinfRR}{{L^\infty(\R;\R)}}
\newcommand{\LoneR}{{L^1(\R)}}
\newcommand{\LoneRR}{{L^1(\R;\R)}}
\renewcommand{\L}[1]{L^{#1}}
\newcommand{\Lloc}[1]{L^{#1}_{loc}}

%Nonlocal look ahead distance for the source term
\newcommand{\nds}{{\nu}}
%Kernel Function for source term
\newcommand{\ws}{W_{\nds}}
%Nonlocal look ahead distance for the transport term
\newcommand{\ndt}{{\eta}}
%Kernel Function for transport term
\newcommand{\wt}{\omega_{\ndt}}
\newcommand{\twt}{\tilde{\wt}}
%Upperbound for discrete convolution
\newcommand{\Ne}{N_\ndt}
\usepackage{ragged2e}

%Kernel Functions transport:
\newcommand{\wtcon}{\wt^{\text{const.}}}
\newcommand{\wtlin}{\wt^{\text{lin.}}}
\newcommand{\wtconcave}{\wt^{\text{conc.}}}
%Coupling function:
\newcommand{\coupling}{g}
\newcommand{\newg}{\Gamma}
%Test functions
\newcommand{\testf}{\phi}

%Discrete rho
\newcommand{\dr}{\rho^{\Dx}}
%N_T Time iterations scheme
\newcommand{\NT}{{N_T}}

%n for different \Dx values for convergence
\newcommand{\nconv}{\mathcal{N}}

%Characteristics
\newcommand{\chr}{X}
%Characteristics of rho, t0, x0
\newcommand{\chrptxz}{{\chr_\rho[t_0,x_0]}}


%Paper Maximum Principle
\renewcommand{\P}{P}
\newcommand{\w}{w}
\newcommand{\coeff}{\mu}
\newcommand\opt{{\text{opt}}}
\newcommand\brho{{\bm{\rho}}}
\renewcommand{\S}{SI}

% quadrature
\newcommand{\qn}{{\nu}}
\newcommand{\nqn}{{J}}
\newcommand{\qw}{{h}}
\newcommand{\qwn}{\qw_\qn}
\newcommand{\qvar}{{y}}

%Order of reconstruction
\newcommand{\g}{o}
\newcommand{\GPopt}{O}


%For networks
\newcommand{\road}{E}
\newcommand{\roadind}{e}
\newcommand{\vertice}{Z}
\newcommand{\verticeind}{z}
\newcommand{\Ro}{\rho^{\max}_1}
\newcommand{\Rt}{\rho^{\max}_2}
\newcommand{\Rtr}{\rho^{\max}_3}
\newcommand{\Rr}{\rho^{\max}_\roadind}
\newcommand{\po}{\rho_1}
\newcommand{\pt}{\rho_2}
\newcommand{\pe}{\rho_\roadind}
\newcommand{\roadbeginohne}{a}
\newcommand{\roadbegin}{\roadbeginohne_\roadind}
\newcommand{\roadendohne}{b}
\newcommand{\roadend}{\roadendohne_\roadind}
\newcommand{\incoming}{\mathcal{I}}
\newcommand{\incomingind}{i}
\newcommand{\NI}{N_\incoming}
\newcommand{\outgoing}{\mathcal{O}}
\newcommand{\outgoingind}{o}
\newcommand{\NO}{N_\outgoing}
\newcommand{\distMatrix}{\mathbb{A}}
\newcommand{\distpar}{\alpha}
\newcommand{\priopar}{q}
\newcommand{\lipschitzcoupling}{{L_\coupling}}
\newcommand{\totaltraveltime}{TTT}
\newcommand{\outflow}{O}
\newcommand{\congestionmeasure}{CM}


\newcommand{\newgo}{\newg_{\outgoingind}}

%Multilane
\newcommand{\borho}{\boldsymbol{\rho}}
\newcommand{\bodr}{\boldsymbol{\rho}^{\Dx}}
\newcommand{\drl}{\rho^{\Dx,\ell}}
\newcommand{\caratt}[1]{{\chi_{\strut#1}}}
\newcommand{\spt}{\mathop{\rm supp}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\boV}{\boldsymbol{V^\nds}}
%Characteristics of bold rho and \ell
\newcommand{\chrl}{\chr_{\borho,\ell}}
\newcommand{\chrb}{\chr_{\borho}}

%GARZ
%Lagrangian marker
\newcommand{\lm}{\omega}
\newcommand{\vg}{u}
\newcommand{\VG}{U}

\newcommand{\jan}[1]{\textcolor{orange}{[Jan: #1]}}
\newcommand{\sudha}[1]{\textcolor{purple}{sudha: #1}}
\newcommand{\rv}[1]{\textcolor{blue}{#1}}
